TRASH: Tandem Rover and Aerial Scrap Harvester

Addressing the challenge of roadside litter in the United States, which has traditionally relied on costly and ineffective manual cleanup methods, this paper presents an autonomous multi-robot system for highway litter monitoring and collection. Our solution integrates an aerial vehicle to scan and gather data across highway stretches with a terrestrial robot equipped with a Convolutional Neural Network (CNN) for litter detection and mapping. Upon detecting litter, the ground robot navigates to each pinpointed location, re-assesses the vicinity, and employs a "greedy pickup" approach to address potential mapping inaccuracies or litter misplacements. Through simulation studies and real-world robotic trials, this work highlights the potential of our proposed system for highway cleanliness and management in the context of Robotics, Automation, and Artificial Intelligence

==> formatting/bibliography-setup.tex <==
\bibliography{ref} 
\bibliographystyle{ieeetr}

==> formatting/do_not_number.tex <==
%include this file in the preamble
%removes numbering from section headings
\setcounter{secnumdepth}{0} % sections are level 1

==> formatting/figures.tex <==
\newcommand{\fig}[3]
    {\begin{figure}
        \centering
        \includegraphics[width=#2in]{#1}
        \caption{#3}
        \label{#3}
     \end{figure}}


\newcommand{\tabl}[2]
    {\begin{table}
        \centering
        {#1}
        \caption{#2}
        \label{#2}
    \end{table}}
    
    
\newcommand{\figref}[1]{(Figure \ref{#1})}

\newcommand{\tableref}[1]{(Table \ref{#1})}

==> formatting/graphics.tex <==
%include this file in the preamble
%Adds images stored in the main file tree
%to use, "\includegraphics{fname.png}[]
\usepackage{graphicx}
\graphicspath{./}

==> formatting/header_footer.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
% \thepage inserts the page number
% [RE, RO] are alignment tabs
% \fancyfoot is also a command 
\fancyhead[RE,RO]{Advertisement Analysis: Surfrider Foundation \thepage}
\renewcommand{\headrulewidth}{0pt}

==> formatting/line_spacing.tex <==
\usepackage{setspace}
%set to 1 for single space, 2 for double space, and so on
\setstretch{1.5}

==> formatting/margins.tex <==
\usepackage[margin=0.5in]{geometry}

==> formatting/table_of_contents_setup.tex <==

%include this file in the preamble
%to use, type in "\tableofcontents" sometime after \begin{document}
\usepackage{color}   %May be necessary if you want to color links
\usepackage{hyperref}
\hypersetup{
    colorlinks=true, %set true if you want colored links
    linktoc=all,     %set to all if you want both sections and subsections linked
    linkcolor=blue,  %choose some color if you want links to stand out
}
